Bayesian Multi--Dipole Modeling of a Single Topography in MEG by Adaptive Sequential Monte Carlo Samplers

In the present paper, we develop a novel Bayesian approach to the problem of estimating neural currents in the brain from a fixed distribution of magnetic field (called \emph{topography}), measured by magnetoencephalography. Differently from recent studies that describe inversion techniques, such as spatio-temporal regularization/filtering, in which neural dynamics always plays a role, we face here a purely static inverse problem. Neural currents are modelled as an unknown number of current dipoles, whose state space is described in terms of a variable--dimension model. Within the resulting Bayesian framework, we set up a sequential Monte Carlo sampler to explore the posterior distribution. An adaptation technique is employed in order to effectively balance the computational cost and the quality of the sample approximation. Then, both the number and the parameters of the unknown current dipoles are simultaneously estimated. The performance of the method is assessed by means of synthetic data, generated by source configurations containing up to four dipoles. Eventually, we describe the results obtained by analyzing data from a real experiment, involving somatosensory evoked fields, and compare them to those provided by three other methods.

==> par_2.tex <==
In the present subsection we recall the key ingredients of a recently developed class of methods, called Sequential Monte Carlo samplers, for approximating a complex probability distribution of interest with a small computational cost. The reader is referred to \cite{dedoja06} for a full description of the subject.
\smallskip

Let us suppose we want sample from a given density $\pi\/(x)$, defined on a state space $\V{}$. We shall express $\pi\/(x)\@$ as the ratio $\g\/(x)\@/\@Z\@$, where $\g \colon \V{} \to \R^+$ is known pointwise while the normalizing constant $Z\@$ may be unknown. 

In most cases, $\@\pi\@$ is complex enough to make direct importance sampling inapplicable. This is because the importance density has to be as much as possible similar to the target density and therefore it is itself not tractable.


A natural way to overcome this issue is by resorting to a sequential version of the importance sampling:
first of all a tempering sequence of distributions $\@\{\@\pi_n\/(x\/)\@\} : = \{\@\g_n\/(x)\@/\@Z_n\@\}$, $n = 1, \ldots, N$,
%all defined on $\V{}\@$ and 
is built in such a way that $\@\pi_1\/(x)\@$ be easy to approximate by means of a sensible importance distribution $\eta_1\/(x)\@$ and $\pi_N\/(x)=: \pi\/(x)\@$ be the target density. Then, at each step, the particle approximation $\@\{X^\narc{i}_{n}\@\}_{\plus62 i=1}^{I}\@$ of $\pi_n\/(x)\@$\vspace{1pt} is moved to the subsequent step by means of 
a Markov kernel $K_n$. However, in most cases, it is impossible to compute the resulting marginal distribution analytically and therefore the standard IS estimate of $\pi_{n+1}\/(x)\@$ is not available.

In the traditional Sequential Importance Sampling (SIS) approach, a pointwise approximation  for $\eta_{n-1}\/(x)\@$ with $I$ particles is thus performed, yielding to
\begin{equation}\label{SIS_part}
 \eta_n\/(x) \sim \frac{1}{I}\, \sum_{i = 1}^I\@ K_n\@(\@X^\narc{i}_{n-1}, x\@).
\end{equation}
This has however a very high computational cost of  $\text{O}\/(I^{\plus02 2})$ as the evaluation of $\eta_n\/(x_n)$ requires $I$ operations for any single particle.


%As an example, in a Bayesian setting, $\@\pi_1\/(x)\@$ is typically the prior distribution, while  $\@\pi_N\/(x)\@$ is the posterior. 

\smallskip
The Sequential Monte Carlo (SMC) sampler addresses this issue at the price of performing importance sampling in an increasingly larger space $\V{}^{\/n} := \underbrace{\V{} \times \cdots \times \V{}}_{n\ times}\@$ whose points $(\/x_1, \ldots, x_n\/)$ will be denoted by $x_{\@1:n}\@$. 

For any $n$, an extended probability distribution $\tilde \pi_n\/(x_{\@1:n}) := \tilde \g_n\/(x_{\@1:n})\@/\@\tilde Z_n$ is introduced, in such a way that its marginal with respect to $x_{1:n-1}$ coincides with $\pi_n\/(x_n)$. 
%
This can be done by introducing artificial backward Markov kernels $\{L_k\}$  
such that $\int_E L_k\/(X_{k+1}, x_k)\@ d\/x_k = 1$ and setting
\[
 \tilde \g_n\/(x_{\@1:n}) = \g_n\/(x_n)\@ \prod_{k = 1}^{n-1}\@ L_k\/(x_{k+1}, x_k)\@.
\]

It is now possible to define, by induction, the following algorithm.

\begin{itemize}
\item For $n= 1$, compute a particle approximation $\big\{X^\narc{i}_1, W^\narc{i}_1\big\}$ of $\pi_1\/(x_1)\@$. As already noticed, the weight function $w_1\/(x_1) = \g_1\/(x_1)\@/\@\eta_1\/(x_1)\@$ can be computed exactly. 
\vspace{3pt}

\item Assuming that at iteration $n-1$
the particle approximation $\big\{X^\narc{i}_{n-1}, W^\narc{i}_{n-1}\big\}$ of $\tilde \pi_{n-1}\/(x_{1:n-1})$ is available, let the path of each particle evolve by means of a Markov kernel $K_n\/(x_{n-1}, x_n)$. The weights now become
\begin{equation*}
\begin{split}
 w_n\/(x_{1:n}) &= \frac{\tilde \g_n\/(x_{1:n})}{\eta_n\/(x_{1:n})} = 
\frac{\g_n\/(x_n)\@ \prod_{k = 1}^{n-1}\@ L_k\/(x_{k+1}, x_k)}{\eta_1\/(x_1)\, \prod_{k=2}^n\@ K_k\/(x_{k-1}, x_k)} = \\[3pt]
&= w_{n-1}\/(x_{1:n-1})\, \frac{\g_n\/(x_n)}{\g_{n-1}\/(x_{n-1})}\, \frac{L_{n-1}\/(x_n, x_{n-1})}{K_n\/(x_{n-1}, x_n)} =\\[3pt]
 &:= w_{n-1}\/(x_{1:n-1})\, \tilde w_n\/(x_{n-1}, x_n)\@.
\end{split}
\end{equation*}
\end{itemize}

Therefore only the ``\@incremental weights\@'' $\tilde w_n\@$ are to be evaluated. As these last are functions of $x_{n-1}$ and $x_n\@$ alone, the computational cost, compared with that of SIS, is sensibly reduced. 

The variance of the (\@unnormalized\@) importance weights tends to increase with $n\@$ and this may lead to a very poor representation of the target density by the sample set. This phenomenon --- called degeneracy --- is routinely measured by using the Effective Sample Size (ESS) criterion. If the degeneracy is too high (e.g. $\text{ESS} < I\@/\@2\@$), it is advisable to perform a resampling step.
%
The SMC sampler may thus be summarized as follows:
\begin{algorithm}
\vspace{2pt}
 \begin{algorithmic}
\State \textbf{set} $n=1$ \Comment{\textit{\underline{Inizialization}}} 
\For{$i=1,\ldots,I$}
\State  draw the particles $X_1^\narc{i} \sim \eta_1$\vspace{1pt}
\State compute $w_1(X_1^\narc{i}) = \gamma_1(X_1^\narc{i})\, /\, \eta_1(X_1^\narc{i})\ \, \forall\ i=1,\ldots,I$\vspace{1pt}
\State normalize $\Rightarrow\@ \{X_1^\narc{i}, W_1^{\narc{i}}\}$
\EndFor
\For{$n=2,\ldots,N$}
\If{$\mathrm{ESS}:=\{\sum_{i=1}^I(W_n^\narc{i})^2\}^{-1}<I\@/\@2\,$} \Comment{\textit{\underline{Resampling}}} \vspace{1pt}
\State resample the particles \vspace{1pt}
\State set $W_n^\narc{i}=1\@/\@N$  
\EndIf
\State \textbf{set} $n = n+1$ \Comment{\textit{\underline{Sampling}}}
\If{$n = N+1$}
\State stop
\Else
\For{$i = 1, \ldots, I$}
\State draw the particles $X_n^\narc{i} \sim K_n(X_{n-1}^\narc{i},\, \cdot\ )$\vspace{2pt}
\State compute $\displaystyle \tilde{w}_n(X^\narc{i}_{n-1\@:\@n})\, =\, 
\frac{\gamma_n(X^\narc{i}_n)\@L_{n-1}(X^\narc{i}_n, X^\narc{i}_{n-1})}{\gamma_{n-1}(X^\narc{i}_{n-1})\@K_n(X^\narc{i}_{n-1}, X^\narc{i}_n)}\ \ \forall\@i=1,\ldots,I$\vspace{2pt}
\State normalize the weights $\displaystyle W^\narc{i}_n\ =\ \frac{W^\narc{i}_{n-1}\@\tilde{w}_n(X^\narc{i}_{n-1\@:\@n})}{\plus90\sum_{j=1}^{I}\@W^\narc{j}_{n-1}\@\tilde{w}_n(X^\narc{j}_{n-1\@:\@n})}\@$
\EndFor
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

\smallskip
In order to put the SMC sampler into practice the user has to properly choose three ingredients: the sequence $\{\pi_n\}$, the Markov kernels $\{K_n\}\@$ and the artificial backward transition kernels $\{L_n\}\@$. We shall discuss in the following which choice is more suited to the MEG inverse problem. 

==> par_2_2.tex <==
According to Eq.\,\eqref{federer}, the inverse problem of MEG can be formalized as follows: given the array $\b:=(\@b^{\/1}, \ldots, b^{\@\Ns}\@)$ of the measures of the magnetic field,
determine the state of the neural currents, namely: the number $\nd$ of dipoles,  their positions (\@i.e., 
the cells $c\@(d)$ where they are located\@), the Cartesian components $u^k\left(c\@(d)\right)$ of their directions, and their strengths $q\left(c\@(d)\right)\@$. 

\smallskip
The analysis made above suggests defining the state space $\X$ of the neural currents as
\[
 \X := \bigcup_{\nd=\@0}^{\nd^\text{\tiny{max.}}}\{\nd\}\times \X\/(\nd),
\]
being $\nd^\text{\tiny{max.}} (\@ \ll \nc)$ the maximum number of dipoles allowed by the model and  $\X\/(\nd)\@$ the state space for a fixed number $\nd$ of dipoles.
This is usually called a \emph{variable--dimension model} \citep{roca04, camory05}.

The space $\X\/(\nd)$ can be, in turn, defined as follows. \ifaoas \linebreak \fi
First of all, $\X\/(\nd):=\emptyset$ for $\nd=0$. Then $\X\/(\nd):=\J$ for $\nd=1$, being $\@\J\/$ the state space  of a single dipole.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
On account of the previous considerations, $\@\J\/$ can be defined as the Cartesian product $\N_{C}\times \mathbb{P}^2\/(\R)\times K$, where $\N_C:=[1,\nc]\cap \N\@$ is the space of cell numbers, the real projective plane $\mathbb{P}^2(\R)$ is the space of dipole directions and $K$ is the space of dipole strengths, which may be either $\R$ or $\C$; in the simulations of Sec. \ref{S_4} and Sec. \ref{S_5}, $K := \R\@$. We recall that $\mathbb{P}^2(\R)$
can be regarded as the quotient space of the $2$--sphere by identifying any two antipodal points. Referring $\R^3$ to cylindrical coordinates $(\rho,\varphi,z)\@$, the Cartesian components of a point $\mathbf{u}$ in $\mathbb{P}^2(\R)$ can thus be expressed as
\begin{equation}\label{ziocil}
 \left\{
\begin{array}{lcl}
  u^{1} & = & \sin(\arccos\/z)\@\cos\/\varphi \\
  u^{2} & = & \sin(\arccos\/z)\@\sin\/\varphi \\
  u^{3} & = & z,
\end{array}
\right.
\end{equation}
with $z\in [0,1]$ and $\varphi\in [0,2\pi)$ if $z\neq 0$, $\varphi\in [0,\pi)$ if $z=0$. 
The two coordinates $z$ and $\varphi$, in the ranges just specified, shall be used  to express the Cartesian components 
(\ref{ziocil}) of the dipole direction $\mathbf{u}$. Summing up, the state of a single dipole will be represented as the point
$j=(c,z,\varphi,q)\in\J$.

To address the case $\nd>1$, the first step is to consider the Cartesian product $\J^{\@\Nd}:=\J\times\ldots\times\J$ of $\nd$ 
copies of $\J$. A point of $\J^{\@\Nd}$ will be denoted by the vector $\big(\@j^\narc{1},\ldots,j^\narc{\nd}\big)$; in turn, 
for $d=1,\ldots,\nd\@$, each $\@j^\narc{d}\@$ is of the form $j^\narc{d}=\big(c^\narc{d},z^\narc{d},\varphi^\narc{d},q^\narc{d}\big)\@$, 
where $q^\narc{d}$ is synonymous with $q\/(\/c\@(d)\/)$ above. Now, for the concept of  ``\@number of dipoles $\nd$\@'' to be well--posed, 
any ambiguous representation of a single dipole as a vector sum of dipoles applied at the same point should be avoided. 
For this reason, the $\nd$ dipoles shall be constrained to be applied at different points. This entails subtracting from $\J^{\@\Nd}$ the set 
\begin{equation}
\J^{\Nd}_{eq.}:=\left\{\big(j^\narc{1},\ldots,j^\narc{\nd}\big)\in\J^{\@\Nd}\,|\, \exists\, i,\,j\in\{1,\ldots,\nd\@\}\, :\, c\@(i)=c\@(j)\right\}
\end{equation}
to obtain the new space 
$\J_{\Nd}:=\J^{\Nd}\setminus \J^{\Nd}_{eq.}$.
Moreover, the \emph{order} in any $\nd\@$--ple $\big(\@j^\narc{1},\ldots,j^\narc{\nd}\big)$ has no actual physical meaning: 
any two $\nd\@$--ples differing only by a permutation of their components $j^\narc{d}$ should then be identified. This amounts to setting onto $\J_{\Nd}$ the equivalence relation induced by the action of the symmetric group $S_{\Nd}$. The resulting quotient 
space $\J_{\Nd} /\!\sim\@$ is eventually the appropriate choice for the space $\X\/(\nd)$. An equivalence class in $\J_{\Nd} /\!\sim\@$ shall be denoted by $\@j_{\Nd}\@$. Note that, for $\nd=0$, $\J_{\Nd} /\!\sim\ =\emptyset$ and, for $\nd=1$, $\J_{\Nd} /\!\sim\ =\J$, which is consistent with the previous settings.

As a result of the above investigation, the state space of neural currents is defined as the following disjoint union:
\begin{equation}\label{eq_spazio_stati}
\X:= \bigcup_{\nd=\@0}^{\nd^\text{\tiny{max.}}}\{\nd\}\times \J_{\Nd} / \sim.
\end{equation}
A point in the space $\X$, i.e., a pair $\big(\@\nd,\@j_{\Nd}\big)$, will be denoted by $x\@$.

